Seedance 1.5 pro: A Native Audio-Visual Joint Generation Foundation Model

Recent strides in video generation have paved the way for unified audio-visual generation. In this work, we present Seedance 1.5 pro, a foundational model engineered specifically for native, joint audio-video generation. Leveraging a dual-branch Diffusion Transformer architecture, the model integrates a cross-modal joint module with a specialized multi-stage data pipeline, achieving exceptional audio-visual synchronization and superior generation quality. To ensure practical utility, we implement meticulous post-training optimizations, including Supervised Fine-Tuning (SFT) on high-quality datasets and Reinforcement Learning from Human Feedback (RLHF) with multi-dimensional reward models. Furthermore, we introduce an acceleration framework that boosts inference speed by over 10X. Seedance 1.5 pro distinguishes itself through precise multilingual and dialect lip-syncing, dynamic cinematic camera control, and enhanced narrative coherence, positioning it as a robust engine for professional-grade content creation. Seedance 1.5 pro is now accessible on Volcano Engine at https://console.volcengine.com/ark/region:ark+cn-beijing/experience/vision?type=GenVideo.

==> sections/Conclusion.tex <==
\label{Conclusion}


\section{Conclusion} 

We have introduced Seedance 1.0, a native bilingual video generation foundation model that unifies multiple generation paradigms (such as text-to-video and image-to-video) and excels in instruction following, motion stability, and visual quality. We presented our technical improvements in dataset construction, efficient architecture design with training paradigm, post-training optimization, and inference acceleration, which are integrated effectively to achieve a high-performance model with fast inference. It demonstrates excellent capabilities in handling complex scenarios, multi-shot generation, and long-range temporal coherence, all while delivering fast and photorealistic generation experiences.
%We hope that seedance 1.0 can pave the way for scalable professional and creative video production.


==> sections/Data.tex <==
\section{Data}
\label{sec:data}

% \begin{figure*}[t]
% \centering
% \includegraphics[width=\textwidth]{figures/data_processing.pdf}
% \caption{}
% \label{fig:data_processing}
% \end{figure*}


\subsection{Data Curation Pipeline}

To construct a dataset capable of high-fidelity audio–visual generation, we design a comprehensive multi-stage data curation pipeline. Compared with the earlier vision-only version, the upgraded pipeline pays more attention to audio–visual coherence, motion expressiveness, and a curriculum-oriented data stage. Each component of the pipeline is listed below in detail.

\textbf{\textit{Holistic Audio–Visual Sourcing.}}
Firstly, we collecting data that captures the full spectrum of interactions between visual dynamics and acoustic environments. The sourcing strategy maintains diversity across subjects, scenes, styles, and motion patterns, while simultaneously ensuring wide coverage of audio modalities. This includes variations in human speech across languages and speaking styles, environmental ambience spanning natural and urban contexts, mechanical and object-induced sound events, and other acoustic cues that tightly correlate with visual motion. The goal is to obtain a balanced corpus in which vision features are matched with equally diverse and representative audio ones.

\textbf{\textit{Audio-Aware Temporal Segmentation.}}
Traditional segmentation pipelines rely solely on visual shot boundaries, which often disrupt coherent audio events. To mitigate this issue, we introduce an audio-aware segmentation mechanism that jointly analyzes visual transitions and short-time acoustic cues. A segment boundary is retained only when visual discontinuities coincide with audio-level evidence, such as a natural pause or a low-activity interval in the soundtrack. This produces clips that preserve semantic continuity in both modalities and ensure that each segment forms a meaningful unit for training audio–visual generation models.

\textbf{\textit{Multimodal Quality Filtering.}}
We apply a rigorous filtering stage to enforce high perceptual quality and safety requirements across both audio and visual channels. Visual quality screening uses a combination of fidelity predictors, aesthetic scoring models, and color consistency metrics. Low-resolution or poorly composed clips are removed. To further improve temporal expressiveness, motion characteristics are evaluated to enable the exclusion of segments with weak, trivial, or uninformative motion.
%
Audio quality is examined through signal-level diagnostics that detect silence, low signal-to-noise ratio, excessive amplification, and other forms of degradation. We use an audio–visual synchronization estimator to measure temporal correspondence between audio and visual actions. Clips exhibiting severe misalignment are discarded to guarantee reliable temporal pairing between modalities.

\textbf{\textit{Joint Audio–Visual Distribution Rebalancing.}}
Large-scale raw collections display substantial long-tail imbalances across both visual and acoustic dimensions. To achieve a well-behaved training distribution, we rebalance the data jointly across visual categories (e.g., object-centric scenes, human-centric activities, and landscape environments) and audio categories (including speech, ambient noise, music, and mechanical or natural sound events). The joint distribution over the Cartesian product of these categories reveals underrepresented combinations that arise infrequently in web-scale data, such as uncommon actions paired with rare environmental acoustics. We increase the sampling weight of such sparse pairs while reducing redundancy among overwhelmingly frequent ones. This recalibration improves the diversity of cross-modal contexts and encourages robust generalization over the full audio–visual manifold.

\textbf{\textit{Curriculum-Based Data Staging.}}
The curated dataset is organized into a multi-stage curriculum designed to gradually strengthen the model’s capacity for audio–visual alignment and generative fidelity. The first stage focuses on enabling the model to acquire fundamental cross-modal correspondence and temporal grounding.
%
The second stage introduces more complex motion patterns, challenging acoustic conditions, multi-speaker or multi-source environments, and scenes where overlapping or rapidly changing sound events occur. As the model progresses through the curriculum, it experiences increasingly difficult audio–visual interactions, ultimately building the ability to synthesize coherent, realistic, and contextually appropriate audio for a wide variety of dynamic visual scenarios.

\subsection{Video Captioning}
\label{sec:caption}

Based on the captioner of Seedance 1.0, we further enhanced the richness of content descriptions, encompassing more detailed depictions of camera movements, actions, and aesthetic elements. Additionally, we have improved the accuracy of shot transition detection and text recognition capabilities. While ensuring accuracy, we also strengthened the professionalism of domain-specific descriptions and the differentiation between descriptions of content with varying quality, tailored to data from different fields.

To enable audio generation, we further added audio descriptions in the caption, covering multiple types such as dialogue, music, and sound effects. Similar to video descriptions, audio descriptions also maintain the richness of content.

We utilized the in-house Seed Omni Model to train our captioner, which possesses strong video understanding,  text recognition and audio recognition capabilities. Simultaneously, we performed quantization acceleration on the model, enabling it to handle annotation for massive volumes of training data.



\subsection{Efficient Engineering Infrastructure}
\label{sec:engineering_infra}

The data pipeline for video generation is required to process multi-modal inputs from videos, images, audio, and text. Sustaining a daily processing throughput of several hundreds of millions imposes stringent requirements on performance optimization.
Firstly, at the resource level, our engineering pipeline is equipped with exceptional flexibility, reflected in its ability to inference with various forms of unstable computing resources. Examples include on-demand preemptive resources, reserved resources available only within specific time windows, and low-cost CPU resources.
Meanwhile, through a well-designed pipeline parallelism mechanism, we achieve high levels of asynchronous parallelism to maximize the utilization of CPUs and GPUs.
Finally, by building automation infrastructure, we minimize human intervention in the data processing workflow, reduce operational dependency and intermediate waiting time, and fully leverage available computing resources.

==> sections/Inference_Acceleration.tex <==
\section{Inference_Acceleration}


==> sections/Model_Design.tex <==
\section{Model Design}


\subsection{Variational Autoencoder}
Variational Autoencoders (VAEs)~\citep{Kingma2013AutoEncodingVB} play a pivotal role in reducing the computational burden of diffusion models by compressing high-dimensional raw signals into compact latent representations, thereby facilitating efficient training and inference. The proposed \model leverages two distinct VAE models to handle multimodal data. Specifically, we adopt the pre-trained 3D video VAE from Seedance 1.0 to compress visual data, and develop a universal audio VAE that efficiently compresses complex audio encompassing speech, sound effects, and music.

\subsection{Diffusion Transformer}
\begin{figure*}[th]
\centering
\includegraphics[width=0.6\textwidth]{figures/model.png}
\caption{The proposed diffusion transformer model of \model.}
\label{fig: model}
\end{figure*}

The proposed diffusion transformer architecture of \model is constructed upon the MMDiT architecture \cite{esser2024scaling}, as illustrated in Figure \ref{fig: model}. To accelerate convergence, the system employs a dual-branch topology. Specifically, we initialize the video branch using weights from the pre-trained Seedance 1.0 Pro model, while the MMDiT-based audio branch is pre-trained from scratch to serve as a robust initialization. To facilitate the synthesis of multimodal representations, we introduce specialized cross-modal joint modules that interconnect the two DiT backbones. During joint training, the video DiT processes visual and textual inputs, while the audio DiT concurrently handles auditory and textual data. The joint modules function as a structural bridge, enabling the effective learning of cross-modality information. During training, the parameters of all modules are trained.

\subsection{Diffusion Refiner}
For high-resolution audio-video generation, we employ a cascaded diffusion framework analogous to Seedance 1.0, distinguished primarily by the integration of an additional audio signal input to support joint generation.


\subsection{Prompt Engineering (PE)}
\label{sec:pe}
The role of the Prompt Engineering model is to understand the content and intention of users' input (user prompt) and convert it into a Caption-style format recognizable by the DiT model. We sampled a large amount of high-quality data from the Continue Training (CT) and Supervised Fine-Tuning (SFT) stages, spanning multiple domains. Based on the caption model, we trained the model to acquire rewriting capabilities for Image-to-Video (I2V) and Text-to-Video (T2V) tasks. To enhance the model's performance in the test time, we manually annotated a batch of data with rich expressiveness and narrative qualities. This enables the model to demonstrate more comprehensive and reasonable creative capabilities under crude and generalized user prompts.

==> sections/Model_Optimization.tex <==
\section{Inference Optimizations}

\subsection{Model Acceleration}
We employ diffusion distillation to expedite DiT inference by lowering the number of required function evaluations (NFE) during generation. Building on the distillation scheme used in Seedance 1.0\cite{gao2025seedance}, we further refine the TSCD pipeline in HyperSD\cite{ren2025hyper} by incorporating meanflow\cite{geng2025mean} distillation strategy. Specifically, we apply multi-segment average-velocity transformations to the original joint video–audio generation trajectories. This design enables our model to perform coupled video–audio generation more efficiently.
To further enhance acceleration, we adopt a score-based distillation scheme inspired by RayFlow \cite{shao2025rayflow}. The student is trained to approximate the teacher’s score via an expected noise-consistency objective, enabling trajectory-level optimization. This yields more reliable sampling at low NFEs and reduces artifacts during fast inference. Finally, a human-preference-guided adversarial training mitigates low-step inference artifacts.Human evaluation confirms that the accelerated model maintains video and audio quality on par with the original.

\subsection{Inference Infrastructure}

% \textbf{High-Performance Kernel.} Extensive kernel fusion efforts have been conducted on the model's core modules, resulting in a cumulative 15\% improvement in the model's inference throughput.

% \textbf{Quantization and Sparse.} Building on the Seedream \cite{gong2025seedream} technical solution, we have implemented fine-grained mixed-precision quantization tailored for Attention and Gemm operations. Moreover, our exploration revealed that the sparse attributes of DiTs exhibit hierarchical and blockified structures across and within various modalities. Expanding on the methodology established by AdaSpa \cite{adaspa}, we have introduced a streamlined tuning solution focused on minimizing search stage overhead. Additionally, we have successfully integrated our optimized fine-grained Attention Quantization approach into this scheme. Numerous efforts have been dedicated to mitigating the impact of full quantization and sparsity on the quality of pixel-level generation. We have achieved an optimal balance between performance and efficiency.

% \textbf{Parallelism Strategy.} In order to decrease the allocated massive memory due to the long sequence in video generation schema. A customized adaptive hybrid parallel strategy has been proposed to effectively split the sequences. This approach integrates the concept of context parallelism to optimize communication processes, resulting in a reduction of communication overhead to a quarter of the level observed in Ulysses \cite{jacobs2023deepspeed}. Simultaneously, we have further reduced end-to-end communication overhead by introducing FP8 communication. 

% \textbf{Async Offloading Strategy.} Due to the extensive computational demands of attention coupled with the large model size. We developed an automated and adaptive AsyncOffloading strategy. We successfully solved the large model deployment problem on memory-limited devices with a performance drop of less than 2\%.

% \textbf{Hybrid Parallelism for Distributed VAE.} Moreover, to address the issue of high GPU memory consumption due to the VAE-Decoder, we implemented an adaptive hybrid parallel strategy. This method partitions the input data along the spatial and temporal dimensions simultaneously and employs efficient collective communication for Conv3D computation. Thus, we further improved parallel scaling performance.

% \textbf{Pipeline Optimizations.} We adopted kernel fusion, quantization, parallelization, continuous batching, prefix caching, and other common techniques to improve the overall throughput of the prompt engineering effectively. Furthermore, to tackle the issue of low encoding efficiency in long videos, we have implemented video encoding acceleration solutions. 

Following Seedance 1.0, we further integrate a suite of proprietary optimization algorithms—including kernel fusion, fine‑grained mixed‑precision quantization, and adaptive sparsity—to enhance the performance of key components across the inference pipeline, such as the DiT, VAE, and prompt‑engineering modules. Tailored hybrid parallelization strategies are applied to both the DiT and VAE models, reducing runtime memory while improving multi‑GPU scaling efficiency. By combining decomposition‑based and fusion‑based computation‑communication overlap techniques, we design a comprehensive topology‑aware overlapping scheme that avoids SM contention and enhances kernel efficiency through carefully tuned granularity. To further reduce communication volume, we introduce an 8‑bit communication strategy co‑designed with a model quantization approach to achieve comparable performance. Additionally, an automatic hardware‑aware asynchronous offloading mechanism is implemented to resolve out‑of‑memory issues on heterogeneous GPU settings. With comprehensive pipeline optimizations, we substantially improve inference throughput, reduce communication and memory overhead, and achieve a significant leap in end-to-end efficiency while maintaining high generation quality.

==> sections/Model_Train.tex <==
\section{Model Training}
As shown in Figure \ref{fig:stage}, we illustrate the training and inference phases of Seedance 1.5. Our training process consists of three sub-stages, including Pre-training, Supervised Fine-Tuning (SFT), and Human Feedback Alignment (RLHF). During inference, the Prompt Engineering model parses the user prompt into audio and visual prompts and then feeds them together into the Audio-Video joint model.


\begin{figure*}[hb]
\centering
\includegraphics[width=\textwidth]{figures/stage.png}
\caption{Overview of training and inference pipeline.}
\label{fig:stage}
\end{figure*}

\subsection{Pre-Training}
To achieve native video-audio joint synthesis, we propose a cross-modality joint-model based on the MMDiT architecture, which facilitates deep cross-modality information interaction, ensuring temporal synchronization and semantic consistency between visual and auditory streams. The pre-training stage employs multi-task joint training on a large-scale mixed-modality dataset, enabling the model to generalize across diverse downstream tasks, including Text-to-Audio-Video (T2AV), Image-to-Audio-Video (I2AV), as well as unimodal video generation (T2V, I2V).

\subsection{Supervised Fine-Tuning (SFT)}

After Pre-Training stage, we conduct a supervised fine-tuning stage (SFT) to further align the model’s generative capabilities with human preferences. Specifically,  targeting improving visual aesthetics, motion coherence, and audio fidelity, we construct a high-quality dataset of audio-visual-text triplets, meticulously curated across hundreds of categories that define specific visual styles, motion dynamics, and acoustic attributes. During the training process, we adopt a refined stepwise annealing strategy. This approach allows us to progressively adjust the learning rate and data distribution, ensuring that the model stabilizes effectively while retaining precise text controllability. Furthermore, to fully leverage high-quality data, we train different expert models on distinct sub-domains and subsequently integrate their strengths via the model merging technique. This combination of curated data, strategic annealing, and parameter fusion significantly enhances the performance of the model, resulting in superior visual quality, fluid motion, and synchronized audio in video generation.
% Following CT, we perform supervised fine-tuning (SFT) to further align the model's output with human preferences regarding visual quality and motion coherence. During this phase, the model trains on a carefully curated set of high-quality video-text pairs with manually verified captions, allowing it to generate videos with improved aesthetics and more consistent motion dynamics.


% \textbf{Human-Curated Dataset.} Ensuring data quality and distributional balance is essential. To achieve this, we define several hundred categories based on visual style, motion type, and other key attributes. We then collect data in a targeted manner within each category, resulting in a curated dataset of high-quality video samples with accurate and meaningful captions.
% %All captions are manually verified to ensure precise alignment with their corresponding videos.


% \textbf{Model Merging.} To fully leverage high-quality data, we train separate models on curated subsets designed to capture a wide range of styles, motions, and scenarios. The resulting models are subsequently merged into a single model that integrates their respective strengths. Each model is trained with a smaller learning rate than in pre-training and utilizes a limited number of GPUs. Moreover, we apply early stopping at an effective point to prevent overfitting and maintain text controllability. The final merging step significantly improves both visual fidelity and motion quality.




\subsection{Human Feedback Alignment (RLHF)}

Reinforcement Learning from Human Feedback (RLHF) has become a pivotal optimization technique in visual generation\cite{liu2025flow,xue2025dancegrpo,wu2025rewarddance,zhang2024unifl}, widely adopted by prominent models such as Qwen-Image\cite{wu2025qwen}, Hunyuan-Video 1.5\cite{wu2025hunyuanvideo}, the Seedream series \cite{gong2025seedream, gao2025seedream, seedream2025seedream}, and Seedance 1.0\cite{gao2025seedance}.
To advance our joint audio-video generation capabilities, we have designed a multi-component reward system comprising three specialized models (RMs): Audio-Video Alignment, Motion Dynamics, and Aesthetics. The annotation process for each RM is meticulously designed to capture fine-grained, domain-specific corresponding sub-dimensions.
Architecturally, the Audio-Video Alignment RM is built upon our in-house Seed Vision-Language Omni Model (mulitimodal VLM), while the Motion Dynamics and Aesthetics RMs follow the established practices of Seedance 1.0. 
Our RLHF optimization strategy is to maximize the aggregate reward score of these three RMs across a range of  generation tasks (e.g., T2V, T2VA, I2VA), thereby holistically enhancing the model's performance across all corresponding qualitative dimensions.
Moreover, targeted infrastructure optimizations to our RLHF pipeline have yielded a nearly 3x improvement in training speed.

% \subsubsection{Feedback Data Infrastructure}

% We collect prompts from training datasets and online users, and perform data balancing and information filtering on prompts to discard duplicate and ambiguous ones. We collect high-quality video data pairs for human preference labeling, including synthetic videos generated by different stages of our model.  Experimental results demonstrate that the incorporation of multiple source visual materials can further enhance the domain capacity of the RM model, expand the preference upper bound of RM, and strengthen generalization capabilities. We adopt a multi-dimensional annotation approach in the labeling process, i.e., selecting the best and worst videos under a specific labeling dimension while ensuring that the best videos are not inferior to the worst ones in other dimensions. 



% \textbf{Prompt System.} We collect prompts from training datasets and online users, and perform data balancing and information filtering on prompts to discard duplicate and ambiguous ones. We built a unified prompt system to support both RM and RLHF. We align the output of the generative model with human preference by using the response of the Reward Model.

% \textbf{Pair Data Sources.} We collect high-quality video data pairs for human preference labeling, including synthetic videos generated by different stages of our model (including Pretrain, SFT, RLHF, etc.) with different Prompt Engineering strategies, as well as part of high-quality videos from training datasets. Our collection encompasses both image-to-video and text-to-video modalities. Experimental results demonstrate that the incorporation of multistage / multiple source visual materials can further enhance the domain capacity of the RM model, expand the preference upper bound of RM, and strengthen generalization capabilities.

% \textbf{Annotation Protocol.} We adopt a multi-dimensional annotation approach in the labeling process, i.e., selecting the best and worst videos under a specific labeling dimension while ensuring that the best videos are not inferior to the worst ones in other dimensions. Additionally, to enhance annotation precision and practicality, we define and annotate the fine-grained sub-tags besides the primary annotation dimensions. This hierarchical structure facilitates data resampling for specific sub-dimensions during training while simultaneously balancing the Reward Model's training data distribution.




% \begin{figure*}[t]
% \centering
% \includegraphics[width=\linewidth]{figures/reward.png}

% \caption{Reward Curves of Different Reward Models During RLHF Training.}
% \label{fig:Reward}
% \end{figure*}

% \subsubsection{Reward Model}

% To comprehensively enhance model performance, we design a sophisticated reward system comprising three specialized reward models: Foundational Reward Model, Motion Reward Model, and Aesthetic Reward Model. These dimension-specific reward models, coupled with video-tailored RLHF optimization strategies, enable comprehensive improvements in multiple aspects of the model capabilities, as illustrated in Figure \ref{fig:Reward}. Foundational reward model focuses on enhancing fundamental model capabilities, such as image-text alignment and structural stability. We employ a Vision-Language Model as the architecture of this reward model. Motion reward model helps to mitigate video artifacts while enhancing motion amplitude and vividness.
% Given that video aesthetics primarily derive from keyframes, we design the aesthetic reward model from image-space input inspired by Seedream \cite{gao2025seedream,gong2025seedream}, with the data source modified to use keyframes from videos. 




% \textbf{Multi-Dimensional Reward System.} 
%  To comprehensively enhance model performance, we design a sophisticated reward system comprising three specialized reward models: Foundational Reward Model, Motion Reward Model, and Aesthetic Reward Model. These dimension-specific reward models, coupled with video-tailored RLHF optimization strategies, enable comprehensive improvements in multiple aspects of the model capabilities, as illustrated in Figure \ref{fig:Reward}.

% \textbf{Foundational Reward Model.} 
% This model focuses on enhancing fundamental model capabilities, such as image-text alignment and structural stability. We employ a Vision-Language Model (VLM) as the reward model, perform supervised fine-tuning via QA-style instruction modeling with binary (yes/no) responses. During inference, we draw insights from generative Reward Model (RM) designs in language models, using the probability of token "yes" as the reward. This methodology effectively leverages the inherent knowledge of pretrained VLM/LLM while benefiting from reward quality improvement through LLM scaling. Notably, we observe Reward Model Scaling phenomenon by expanding the reward model's parameter scale.

% \textbf{Motion Reward Model.} To circumvent the computational bottleneck of VAE decoding in video-space processing, we propose a latent-space reward model operating directly on VAE-encoded representations. This efficient design is realized by fine-tuning a pre-trained VLM on annotated data, enabling precise discrimination of motion quality from latent space features. Experimental results demonstrate its effectiveness in mitigating video artifacts while enhancing motion amplitude and vividness.

% \textbf{Aesthetic Reward Model.} Given that video aesthetics primarily derive from keyframes, we design an image-space input architecture inspired by Seedream2.0, with the data source modified to use keyframes extracted from videos. Prompts are also input into this aesthetic reward model to encourage prompt-aware aesthetic evaluation and prevent shortcut learning to specific preferences.


% \subsubsection{Base Model Feedback Learning}
% Reward feedback learning  \cite{xue2025dancegrpo,zhang2024onlinevpo,liu2025flow,liu2025improving} have been widely used in currnet diffusion models. In Seedance 1.0, we simulate the video inference pipeline during training, directly predict $x_0$ (generated clean video) when the Reward Model (RM) adequately assesses video quality. The optimization strategy directly maximizes the composite rewards from multiple RMs. Comparative experiments against DPO/PPO/GRPO demonstrate that our reward maximization approach is the most efficient and effective approach, comprehensively improving text-video alignment, motion quality, and aesthetics. Furthermore, we preform multi-round iterative learning between the diffusion model and RMs. This approach raises the performance bound of the RLHF process and is more stable and controllable than dynamic update of the RM.

% \textbf{Video-Centric Feedback Algorithm.}
% We simulate the video inference pipeline during training, directly predict $x_0$ (generated clean video) when the Reward Model (RM) adequately assesses video quality. Subsequently, i) frames are extracted from the video and fed into an Image-based Reward Model for reward calculation; ii) video clips are extracted and input into a Video-space RM for reward calculation. The optimization strategy directly maximizes the composite rewards from multiple RMs. Comparative experiments against DPO/PPO/GRPO demonstrate that our reward maximization approach is the most efficient and effective approach.

% \textbf{Feedback Optimization Strategy.}
% Our enhanced method optimizes sampling timesteps and employ a weight moving average strategy, eliminating conventional constraints like pretraining loss regularization or KL-divergence penalties while comprehensively improving text-video alignment, motion quality, and aesthetics. Under sequence parallelism, we implement frame-wise distributed sampling across GPUs to prevent over-optimization of identical frames. Task-specific reward selection is applied in the training process, for instance, image-to-video (I2V) tasks prioritize source consistency over aesthetic enhancement, thus excluding the Aesthetic Reward Model.

% \textbf{Multi-Round Iterative Learning.}
% We establish cyclic co-optimization between the diffusion model and RMs: initially optimizing the diffusion model, then enhancing RMs based on current generation weaknesses, followed by further diffusion optimization. This approach raises the performance bound of the RLHF process and is more stable and controllable than dynamic update of the RM.


% \subsubsection{Super-Resolution RLHF Framework}
% As shown in Figure \ref{fig:sr_compare}, we also apply RLHF on our diffusion refiner, which can be regarded as a diffusion-based conditional generative model. During training, low-resolution VAE latent space representations serve as conditional inputs to the super-resolution model, while the generated high-resolution videos are evaluated by multiple Reward Models. We directly maximize a linear combination of these reward signals. Notably, our approach applies RLHF directly to the accelerated refiner model, effectively enhancing motion quality and visual fidelity in low-NFE scenarios while maintaining computational efficiency.


%\subsection{Refiner}





% \begin{figure*}[h]
% \centering
% \includegraphics[width=0.95\linewidth]{figures/sr_compare.png}
% \vspace{-5pt}
% \caption{Visualization during different resolutions and RLHF process.}
% \label{fig:sr_compare}
% \vspace{-5pt}
% \end{figure*}


==> sections/infrastructure.tex <==
\iffalse

\section{Training Infrastructure}

This subsection introduces the key strategies for efficient model training，including large-scale pre-training and post-training. First, we employ a parallelism strategy to train the lite model on long-context videos. Second, a Runtime Balance strategy is proposed to address computational imbalance during joint image-video training. Additionally, we design Multi-Level Activation Checkpointing (MLAC) to reduce GPU memory usage and recomputation overhead. Finally, we optimize GPU utilization by implementing fused CUDA kernels to streamline fragmented I/O operations. As a result, out lite model attains a model FLOPs Utilization (MFU) of 38\% in large-scale training with thousands of GPUs.
\subsection{Large-Scale Pre-Training Optimization}
\begin{figure}[h!]
  \centering
  \includegraphics[width=.8\linewidth]{figures/training_infrastructure/runtime_balance.png}
  \caption{Balance samples within one batch across GPUs by runtime metric.
        \textbf{Top}: seqlen-to-runtime lookup table.
        \textbf{Bottom left}: One batch samples across GPUs before balance.
        \textbf{Bottom left}: One batch samples across GPUs after balance.}
  \label{fig:runtime_balance}
\end{figure}

\paragraph{Parallelism Strategy.}
We use 3D parallelism that includes data parallelism, context parallelism, and model sharding to support efficiently distributed training with long-context samples. FSDP~\citep{zhao2023pytorch} shards the model parameters, optimizer states, and gradients across GPUs, and enables overlap between computation and communication to reduce communication overhead and improve distributed training efficiency. We adopt Ulysess~\citep{jacobs2023deepspeed} as our context-parallelism strategy, which iteratively shards samples across the sequence dimension and the head dimension in token-dependent/independent layers through all-to-all communication.
\paragraph{Runtime Balance.}
Joint training of images and videos causes significant computational imbalance across GPUs, leading to inter-device synchronization overhead and reduced training throughput. Existing methods~\citep{ma2025step} based on seqlen (sequence length) and FLOPs fail to achieve optimal balance due to the non-linear relationship between training runtime and these metrics, influenced by varying operator efficiency. To address this, we propose Runtime Balance (\Cref{fig:runtime_balance}), which constructs an offline lookup table mapping seqlen to actual runtime. During training, the process gathers runtime estimates obtained via table queries from all ranks and employs a greedy algorithm to determine the global workload distribution. After that, ranks exchange training samples via communication based on the balancing results to achieve optimal load balance. Notably, runtime balancing is restricted within the same batch to preserve data consistency. To minimize training overhead, proactive balancing for the next batch is performed asynchronously in a sub-process to avoid waiting for the main training process.

\begin{figure}[h!]
  \centering
  \includegraphics[width=\linewidth]{figures/training_infrastructure/mlao.png}
  \caption{Multi-level activation checkpointing(MLAC). (a) Vanilla AC saves inputs on device could still encounter GPU OOM. (b) MLAC further supports offloading module inputs to achieve zero-activation AC, (c) and minimize recomputation overheads by saving compute-bound activations to multi-level storage space.}
  \label{fig:mlao}
\end{figure}
\paragraph{Multi-Levels Activation Checkpointing.}
Activation checkpointing~\citep{chen2016training} introduces significant recomputation overhead during backpropagation and may still encounter GPU OOM issues in long-context scenarios, as it inevitably requires caching the input tensor of the wrapped module. We introduce Multi-Level Activation Checkpointing (MLAC), as shown in \Cref{fig:mlao}, a method for selectively saving any intermediate activation during forward pass on multiple levels of storage, such as GPU, CPU, and disk memory. MLAC minimizes recomputation overhead during backpropagation by prioritizing the caching of output tensors from compute-bound operations. Furthermore, it supports offloading input tensors of the gradient checkpointing module on the CPU and disk to attain zero
activation occupancy in GPU memory, which allows training larger models with longer context.
MLAC incorporates an efficient asynchronous caching and prefetching mechanism that optimizes the overlap between memory transfers and forward/backward computations. Compared to vanilla AC, MLAC makes full use of the available hardware resources and significantly improves training efficiency.

\paragraph{Fused Kernel.}
IO-bound operations such as normalization and RoPE (rotary position encoding) frequently access memory, preventing the Tensor/CUDA core from being fully utilized. 
We introduce kernel fusion techniques that leverage registers and shared memory to store intermediate results from consecutive memory-access-intensive operators and fuse them into a single CUDA kernel. These fused kernels reduce the global memory accesses to one-tenth of the baseline, significantly improving the kernel's arithmetic intensity. Specifically, we fuse QK-Norm, RoPE, and all the attention preprocessing operations and implement the corresponding forward and backward fused kernels. Similar optimization strategies are applied to the rest of the memory-access-intensive operators in the model to improve the training and inference efficiency.

\fi

\section{Training Infrastructures}
To enable efficient large-scale pre-training of the DiT model, we design a highly
optimized training system that emphasizes hardware efficiency, scalability, and robustness. The key components
are summarized as follows.
Parallelism and Memory Optimization. We employ Hybrid Sharded Data Parallelism (HSDP) to efficiently
shard weights and support large-scale training without resorting to tensor or expert parallelism. Memory
usage is optimized through timely release of hidden states, activation offloading, and enhanced FSDP support,
enabling training of large models within available GPU resources.
Kernel and Workload Optimization. Performance-critical operations are accelerated by combining torch.compile
with handcrafted CUDA kernels and operator fusion, reducing redundant memory access. To address workload
imbalance from variable sequence lengths, we introduce a global greedy sample allocation strategy with
asynchronous pipelines, achieving more balanced per-GPU utilization.
Fault Tolerance. Multi-level fault tolerance is built into the system, including periodic checkpointing of model,
optimizer, and dataloader states, pre-launch health checks to exclude faulty nodes, and reduced initialization
overhead. These measures ensure stability and sustained throughput during long-term distributed training.
